In-flight Calibration of Hitomi Soft X-ray Spectrometer (3) Effective Area

We present the result of the in-flight calibration of the effective area of the Soft X-ray Spectrometer (SXS) onboard the Hitomi X-ray satellite using an observation of the Crab nebula. We corrected for the artifacts when observing high count rate sources with the X-ray microcalorimeter. We then constructed a spectrum in the 0.5-20 keV band, which we modeled with a single power-law continuum attenuated by an interstellar extinction. We evaluated the systematic uncertainty upon the spectral parameters by various calibration items. In the 2-12 keV band, the SXS result is consistent with the literature values in flux (2.20 $\pm$ 0.08) $\times$10$^{-8}$ erg s$^{-1}$ cm$^{-2}$ with a 1$\sigma$ statistical uncertainty) but is softer in the power-law index (2.19 $\pm$ 0.11). The discrepancy is attributable to the systematic uncertainty of about $+$6/$-$7% and $+$2/$-$5% respectively for the flux and the power-law index. The softer spectrum is affected primarily by the systematic uncertainty of the Dewar gate valve transmission and the event screening.

==> Makefile <==
# Time-stamp: <Wed Jul 19 06:17:03 JST 2017>

############################################################
# ソースファイル
############################################################
# ソースファイル（必須）
SRC	= ms.tex
# 差分を比較するファイル
SRC_ORIG= $(ARCHDIR)/20180104/$(SRC)


############################################################
# 書式の設定（必須）
############################################################
# Various switches. Choose "yes" or "no".
PDFTEX	= no	# "yes" for pdftex, "no" for dvitex.
A4	= yes	# "yes" for A4, "no" for US Letter.
TEXLIVE = yes	# "yes" for Japanese, "no" for English.
LNDSCP	= no	# "yes" for landscape, "no" for portrait.

# Journal and proposal selection. Choose one of these.
PASJ	= yes	# PASJ
AAS	= no	# ApJ, ApJS, ApJL, AJ, PASP
AAP	= no	# A&A, A&AL
MNRAS	= no	# MNRAS


############################################################
# コンパイルの設定
############################################################
BIBFILES= crab.bib sxs_spie.bib sxs_jatis.bib sxs_pasj.bib
compile-prehook:
#	@for i in $(BIBFILES) ; do \
#	$(CAT) $${i} $(BIBTOOL) -s > $${i}_tmp ;\
#	$(MV) $${i}_tmp $${i} ;\
#	done
#	$(CAT) $(BIBFILES) > ms.bib

compile-posthook:
#       pdftk jaxa_sxs_memo_2011_025.pdf a2.pdf a3.pdf output jaxa_sxs_memo_2011_025a.pdf


############################################################
# アップロードの設定
############################################################
# アップロード先のディレクトリ
UPLOADDIR	= /home/astro/public_html/ft/okajima/20170404_eH6yuiwIpwD8RaRzwKcsArPvHpjIYzbioVcc5go819dva4V5nFq8WkSnGghSFDGi
# アップロードする追加ファイル（コンパイルに必要なファイルは自動で含まれる）
UPLOADFILES	= ms_diff*.pdf review*
# アップロード時に追加で実行するコマンド
upload-hook:
	@$(ECHO) '${HOME}/public_html/ft/.fetch.sh up'


############################################################
# バックアップの設定
############################################################
# バックアップ先のディレクトリ
BACKUPDIR	= ./$(ARCHDIR)/$(DATE_TAG)
# バックアップする追加ファイル（コンパイルに必要なファイルは自動で含まれる）
BACKUPFILES	=
# サブミット時に追加で実行するコマンド
backup-hook:


############################################################
# コマンド設定（変更不要）
############################################################
MAKEFILEDIR	= /usr/local/xray/Makefiles
include		${MAKEFILEDIR}/Makefile

